Exact Spike Train Inference Via $\ell_0$ Optimization

In recent years, new technologies in neuroscience have made it possible to measure the activities of large numbers of neurons simultaneously in behaving animals. For each neuron, a fluorescence trace is measured; this can be seen as a first-order approximation of the neuron's activity over time. Determining the exact time at which a neuron spikes on the basis of its fluorescence trace is an important open problem in the field of computational neuroscience. Recently, a convex optimization problem involving an $\ell_1$ penalty was proposed for this task. In this paper, we slightly modify that recent proposal by replacing the $\ell_1$ penalty with an $\ell_0$ penalty. In stark contrast to the conventional wisdom that $\ell_0$ optimization problems are computationally intractable, we show that the resulting optimization problem can be efficiently solved for the global optimum using an extremely simple and efficient dynamic programming algorithm. Our R-language implementation of the proposed algorithm runs in a few minutes on fluorescence traces of $100,000$ timesteps. Furthermore, our proposal leads to substantial improvements over the previous $\ell_1$ proposal, in simulations as well as on two calcium imaging data sets. R-language software for our proposal is available on CRAN in the package LZeroSpikeInference. Instructions for running this software in python can be found at https://github.com/jewellsean/LZeroSpikeInference.

==> bak-intro-v6.tex <==
% !TEX root = ms.tex

\section{Introduction}
\label{sec:intro}

 
  When  a neuron spikes, calcium floods the cell. 
   In order to quantify intracellular calcium levels, calcium imaging techniques make use of 
    fluorescent calcium indicator molecules \citep{dombeck2007imaging,ahrens2013whole,prevedel2014simultaneous}. 
    Thus, a  
  neuron's 
  \emph{fluorescence trace} can be seen as a first-order approximation of its activity level over time.

  
  
    However, the fluorescence trace itself is typically not of primary scientific interest: 
     instead, it is of interest to determine the underlying neural activity, that is, the specific times at which the neuron spiked. 
  Inferring the spike times on the basis of a fluorescence trace
   amounts to a challenging  deconvolution problem, which has been the focus of substantial investigation
 \citep{grewe2010high,pnevmatikakis2013bayesian,theis2016benchmarking,deneux2016accurate,sasaki2008fast,vogelstein2009spike,yaksi2006reconstruction,vogelstein2010fast,holekamp2008fast, friedrich2016fast, friedrichfast2017}. 
 In this paper, we propose a new approach for this task, which is based upon the following insight:  an auto-regressive model for calcium dynamics considered  by \cite{vogelstein2010fast}, \cite{friedrich2016fast}, and \cite{friedrichfast2017} leads directly to a simple $\ell_0$ optimization problem, for which an efficient and exact algorithm is available.
 
\subsection{An Auto-Regressive Model for Calcium Dynamics} 

In this paper, we consider an auto-regressive model for calcium dynamics that has been extensively studied in the recent literature \citep{vogelstein2010fast,friedrich2016fast,friedrichfast2017,pnevmatikakis2016simultaneous}. %We begin by reviewing the model of \cite{vogelstein2010fast}.


\cite{vogelstein2010fast} proposed that  
 $y_t$, the fluoresence at the $t$th timestep, is a noisy realization of $c_t$, the calcium concentration at the $t$th timestep. In the absence of spikes, the calcium concentration decays exponentially according to a first-order auto-regressive process, with decay parameter $0<\gamma<1$. A spike at the $t$th timestep causes the calcium concentration to increase. Letting $z_t$ denote the number of spikes at the $t$th timestep, this leads to the model %This leads to the model 
\begin{align}
& y_t = \beta_0  + \beta_1 c_t + \epsilon_t,   \nonumber\\
& c_t = \gamma c_{t-1} + z_t,  \nonumber\\
& \epsilon_t \sim_\text{ind.} N(0, \sigma^2), \nonumber  \\
& z_{t} \sim_\text{ind.} \mathrm{Pois}(\theta),  \quad t = 1, \ldots, T.
\label{eq:jovo-model}
\end{align}
Note that the quantity $y_t$  in \eqref{eq:jovo-model} is observed; all other quantities  are unobserved. % Here
  The parameter of interest is $z_t$,  the number of spikes that occurs at the $t$th timestep. 
   Figure~\ref{fig:overshrink}(a) displays a small dataset generated according to \eqref{eq:jovo-model}. 
   

  
 
 In what follows, for ease of exposition, we assume $\beta_0=0$ and $\beta_1=1$ in \eqref{eq:jovo-model}. This assumption results in no loss of generality, since $\beta_0$ and $\beta_1$ can be estimated from the data, and $y_1,\ldots,y_T$ can be centered and scaled accordingly.  Furthermore, all results in this paper allow for general $\beta_0$ and $\beta_1$. See Section~\ref{sec:extensions} for additional details.
 
Unfortunately, maximum a posteriori (MAP) inference for $z_{t}$ in  \eqref{eq:jovo-model} is computationally intractable. This led  \cite{vogelstein2010fast} to approximate the Poisson distribution in \eqref{eq:jovo-model} with an exponential distribution.  They argued that 
under this approximation, the MAP estimate of $z_t$ in \eqref{eq:jovo-model}
is  equivalent 
%\textcolor{red}{I'm writing ``equivalent" instead of ``identical", and also I softened the wording, b/c I'm not quite sure that the exponential distribution approximatoin to \eqref{eq:jovo-model} leads EXACTLY to \eqref{eq:convex}, and I want to make sure not to write anything that isn't true. what do you think??}
  to the value of $s_t$ that solves the  $\ell_1$, or  \textcolor{red}{you were missing $s_1,\ldots,s_T$ under `minimize'}
   \emph{lasso} \citep{ti96}, problem  %of the form %\eqref{eq:convex} 
  \begin{equation}
\minimize{c_1,\ldots,c_T,s_2,\ldots,s_T}{  \frac{1}{2} \sum_{t=1}^T \left( y_t - c_t \right)^2 + \lambda \sum_{t=2}^T | s_t |} \mbox{ subject to } s_t = c_t - \gamma c_{t-1} \geq 0, 
   \label{eq:convex}
   \end{equation}
where the nonnegative tuning parameter $\lambda$ equals $\sigma^{2}\theta$. In moving from \eqref{eq:jovo-model} to \eqref{eq:convex}, we replace $z_{t}$ with $s_{t}$ in order to  emphasize a difference in interpretation: $z_t$ takes on integer values, and thus can be interpreted as the number of spikes  at the $t$th timestep; by contrast, since $s_t$ is continuous-valued,  rather than interpreting it as the number of spikes, we instead interpret a positive $s_t$ to indicate the presence of at least one spike at the $t$th timestep, and a zero $s_t$ to indicate the absence of spikes.   
%In  \eqref{eq:convex}, the squared error loss arises from the assumption that the error terms in \eqref{eq:jovo-model} are normally distributed, the $\ell_1$ penalty arises from the  exponential approximation for the spikes, and the constraint enforces the auto-regressive dynamics for the calcium concentration. 
We note that problem \eqref{eq:convex} is closely-connected to the well-known fused lasso signal approximator \cite{tsrz2005}. 


In more recent work, \cite{friedrich2016fast} and \cite{friedrichfast2017} consider a slight modification to \eqref{eq:convex} by including an additional $\ell_{1}$ penalty for the initial calcium concentration,
     \begin{equation}
\minimize{c_1,\ldots,c_T,s_2,\ldots,s_T}{  \frac{1}{2} \sum_{t=1}^T \left( y_t - c_t \right)^2 + \lambda |c_{1}| + \lambda \sum_{t=2}^T | s_t |} \mbox{ subject to } s_t = c_t - \gamma c_{t-1} \geq 0. 
   \label{eq:convex-fried}
   \end{equation}
   Both   \eqref{eq:convex} and \eqref{eq:convex-fried} are convex optimization problems, for which a well-developed set of optimization algorithms is available \citep{boydconvex,elemstatlearn,hastie2015statistical,bien2016penalized}. 
 In their paper,  \cite{friedrich2016fast} develop a very fast exact algorithm for solving the problem \eqref{eq:convex-fried}, and \cite{friedrichfast2017} develop an
 algorithm for solving  the extension of \eqref{eq:convex-fried} for auto-regressive models of order $p\geq 1$.

In this paper, we take a careful look at the optimization problem \eqref{eq:convex}. While \eqref{eq:convex} was originally motivated by \cite{vogelstein2010fast} as an approximation to the MAP estimate in the model \eqref{eq:jovo-model}, it can be  more directly motivated by way of the simple model
%viewed more directly as  an $\ell_{1}$-regularized regression problem corresponding to the model 
\begin{equation}
 y_t = \beta_0  + \beta_1 c_t + \epsilon_t, \quad 
 c_t = \gamma c_{t-1} + s_t, \quad t = 1, \ldots, T, 
\label{eq:model}
\end{equation}
where $s_t$ is assumed to be sparse and nonnegative; once again, $s_t=0$ indicates the absence of a spike at the $t$th timestep, and $s_t>0$ indicates the presence of at least one spike. Once again setting $\beta_0=0$ and $\beta_1=1$, 
problem \eqref{eq:model} leads directly to the non-convex optimization problem 
   \begin{equation}
\minimize{c_1,\ldots,c_T,s_2,\ldots,s_T}{  \frac{1}{2} \sum_{t=1}^T \left( y_t - c_t \right)^2 + \lambda \sum_{t=2}^T 1_{\left( s_t \neq 0 \right) }} \mbox{ subject to } s_t = c_t - \gamma c_{t-1} \geq 0,
   \label{eq:nonconvex-pis1}
   \end{equation}
   where $1_{(A)}$  is an indicator variable that equals $1$ if the event $A$ holds, and $0$ otherwise.  In \eqref{eq:nonconvex-pis1}, $\lambda$ is a non-negative tuning parameter that controls the number of timesteps at which a spike occurs. 
  Then \eqref{eq:convex} is simply the convex relaxation of \eqref{eq:nonconvex-pis1}, obtained by replacing the non-convex $\ell_0$ penalty with a convex $\ell_1$ penalty. 

%Then \eqref{eq:convex} represents the trade-off, controlled by the tuning parameter $\lambda$, between how closely the  calcium $c_{t}$ agrees with the observed fluorescence $y_{t}$, and the magnitude of  $|s_{t}|$ (which is a convex surrogate for the sparsity of $s_1,\ldots,s_T$). 
% In this view, \eqref{eq:convex} can be seen as a convex relaxation of the optimization problem 
%   \begin{equation}
%\minimize{c_1,\ldots,c_T,s_2,\ldots,s_T}{  \frac{1}{2} \sum_{t=1}^T \left( y_t - c_t \right)^2 + \lambda \sum_{t=2}^T 1_{\left( s_t \neq 0 \right) }} \mbox{ subject to } s_t = c_t - %\gamma c_{t-1} \geq 0,
%   \label{eq:nonconvex-pis1}
%   \end{equation}
%   where $1_{(A)}$  is an indicator variable that equals $1$ if the event $A$ holds, and $0$ otherwise.  In \eqref{eq:nonconvex-pis1}, $\lambda$ is a non-negative tuning %parameter that controls the number of timesteps at which a spike occurs. 
   
The optimization problem \eqref{eq:nonconvex-pis1} 
    is highly non-convex, due to the presence of the indicator variable.  
    In the statistics literature, this term is known as an $\ell_0$ penalty. It is well-known that optimization 
    involving $\ell_0$ penalties is typically computationally intractable: in general, no efficient algorithms are available to solve for the global optimum. 
    By contrast,  \eqref{eq:convex} and \eqref{eq:convex-fried} are convex optimization problems that can be efficiently solved for the global optimum. 

    



\subsection{Contribution of This Paper}
\label{subsec:contributions}

We reiterate here that the optimization problems \eqref{eq:convex} and \eqref{eq:convex-fried}, studied by \cite{vogelstein2010fast}, \cite{friedrich2016fast}, and \cite{friedrichfast2017}, can be seen as convex relaxations of the $\ell_0$ optimization problem \eqref{eq:nonconvex-pis1}, which follows directly from the model \eqref{eq:model}. 
 In other words, under the model \eqref{eq:model}, \eqref{eq:nonconvex-pis1} is the ``right" optimization problem to be solving; 
 \eqref{eq:convex} and \eqref{eq:convex-fried}  are simply computationally tractable approximations to this problem. 
  (In fact,  \cite{friedrichfast2017} allude to this in the ``Hard shrinkage and $\ell_{0}$ penalty'' section of their paper.)  
%Whereas \eqref{eq:nonconvexpis1} is highly non-convex, and seemingly computationally intractable,   \eqref{eq:convex} and \eqref{convex-fried} are convex optimization problems that can be efficiently solved for the global optimum. 
 
 
However, using an $\ell_1$ norm to approximate an $\ell_0$ norm comes with computational advantages at the expense of substantial performance disadvantages: in particular, the use of an $\ell_1$ penalty tends to \emph{overshrink} the fitted estimates \citep{adaptivelasso06}.  This can be seen quite clearly in Figures~\ref{fig:overshrink}(c) and \ref{fig:overshrink}(d). % that the $\ell_1$ problem \eqref{eq:convex-fried} does indeed overshrink the fitted estimates, relative to the $\ell_0$ problem \eqref{eq:nonconvex-pis1}. 

%However, the performance of the $\ell_{1}$ problem for spike event estimation is significantly improved by post-thesholding $s_{t}$ to determine spike events; this is explored in detail in Section~\ref{sec:comparison-methods}.

\textcolor{red}{ I want to remove panel (e) of Figure 1!!!}
  
  \textcolor{red}{could you please re-order the panels in Figure 1 so that they match up with the order in which we discuss them in the text: first a, then c, then d, then b? (And delete e!!!)}
  
\begin{figure}[h]
\begin{center}
(a) \hspace{25mm} (b) \hspace{25mm} (c) \hspace{25mm} (d) \hspace{25mm} (e) \hspace{10mm}
\includegraphics[scale = 0.55,clip]{overshrinkage}
\caption{A toy simulated data example. In each panel, the $x$-axis represents time. Observed fluorescence values are displayed in (\protect\includegraphics[height=0.4em]{grey-circle}). 
\emph{(a)}: Unobserved calcium concentrations  (\protect\includegraphics[height=0.4em]{darkgreen}) and true spike times  (\protect\includegraphics[height=0.4em]{green+}). \emph{(b)}: Estimated calcium concentrations (\protect\includegraphics[height=0.4em]{blue}) and spike times (\protect\includegraphics[height=0.4em]{blue+}) that result from solving the $\ell_0$ optimization problem \eqref{eq:nonconvex-nopos}. \emph{(c)}: Estimated calcium concentrations (\protect\includegraphics[height=0.4em]{red}) and spike times (\protect\includegraphics[height=0.4em]{red+}) that result from solving the $\ell_1$ optimization problem \eqref{eq:convex-fried} with the value of $\lambda$ that yields the true number of spikes. This value of $\lambda$ leads to very poor estimation of both the underlying calcium dynamics and the spikes. 
\emph{(d)}: Estimated calcium concentrations (\protect\includegraphics[height=0.4em]{purple}) and spike times (\protect\includegraphics[height=0.4em]{purple+}) that result from solving the 
 $\ell_1$ optimization problem \eqref{eq:convex-fried} with the largest value of $\lambda$ that results in at least one estimated spike within the vicinity of each true spike. This value of $\lambda$ 
  results in 19 estimated spikes, which is far more than the true number of spikes. The poor performance of the $\ell_1$ optimization problem in panels (c) and (d) is a consequence of the fact that the $\ell_1$ penalty performs shrinkage as well as spike estimation; this is discussed further in Section~\ref{subsec:contributions}. \textcolor{red}{remove: (e) Post-thresholding spikes (\protect\includegraphics[height=0.4em]{darkred+}) that results from solving the $\ell_{1}$ problem with small $\lambda$ and threshold set to yield four spikes. Since the estimated calcium is not well-defined after post-thresholding we cannot plot the estimated calcium concentration.}}
\label{fig:overshrink}
\end{center}
\end{figure}



   
In this paper, we consider a slight modification of \eqref{eq:nonconvex-pis1} that results from removing the positivity constraint,
  \begin{equation}
\minimize{c_1,\ldots,c_T,s_2,\ldots,s_T}{  \frac{1}{2} \sum_{t=1}^T \left( y_t - c_t \right)^2 + \lambda \sum_{t=2}^T 1_{\left( s_{t} \neq 0\right) }} \mbox{ subject to } s_t = c_t - \gamma c_{t-1}. 
   \label{eq:nonconvex-nopos}
   \end{equation}
In practice, the distinction between the problems \eqref{eq:nonconvex-nopos} and \eqref{eq:nonconvex-pis1} is quite minor: on real data applications, for appropriate choices of the decay rate $\gamma$, the solution to \eqref{eq:nonconvex-nopos} tends to satisfy the constraint in \eqref{eq:nonconvex-pis1}, and so the solutions are identical. 

   
Like problem \eqref{eq:nonconvex-pis1}, solving problem \eqref{eq:nonconvex-nopos} for the global optimum appears, at a glance, to be computationally intractable --- we (the authors) are only aware of a few $\ell_0$ optimization problems for which exact solutions can be obtained via efficient algorithms!  
 
 However, in this paper, we show that in fact, \eqref{eq:nonconvex-nopos} is a rare $\ell_0$ optimization problem that can be \emph{exactly solved for the global optimum using an efficient algorithm}. 
  This is because \eqref{eq:nonconvex-nopos} can be seen as a changepoint detection problem, for which efficient algorithms that run in no more than $\mathcal{O}(T^2)$ time, and often closer to $\mathcal{O}(T)$ time, are available. 
  Furthermore, our implementation of the exact algorithm for solving \eqref{eq:nonconvex-nopos} yields excellent results relative to the convex approximation  \eqref{eq:convex-fried} considered by \cite{friedrich2016fast} and \cite{friedrichfast2017}. 
   This vastly improved performance can be seen in Figure~\ref{fig:overshrink}(b).
       
   The rest of this paper is organized as follows. In Section~\ref{sec:algorithm}, we present an exact algorithm for solving the $\ell_0$ problem \eqref{eq:nonconvex-nopos}. 
   In Section~\ref{sec:simulation}, we investigate the performance of this algorithm, relative to the  algorithm of \cite{friedrich2016fast} and \cite{friedrichfast2017} for solving the $\ell_1$ problem \eqref{eq:convex-fried}, in a simulation study. In Section~\ref{sec:realdata}, we investigate the performances of both algorithms for spike train inference on a data set for which the true spike times are known 
   \citep{chen2013ultrasensitive, genie2015} and on a data set from the Allen Brain Observatory \citep{allenStimulusSet2016, hawrylycz2016inferring}. In Section~\ref{sec:extensions} we generalize the problem \eqref{eq:nonconvex-nopos} in order to allow for efficient estimation of an intercept term, and to accommodate an auto-regressive model of order $p>1$ \eqref{eq:model}. Finally, we close with a discussion in Section~\ref{sec:discussion}.  Technical details and additional  results can be found in the Appendix.
   
   
  
  
 
